Wolves in the Repository: A Software Engineering Analysis of the XZ Utils Supply Chain Attack

The digital economy runs on Open Source Software (OSS), with an estimated 90\% of modern applications containing open-source components. While this widespread adoption has revolutionized software development, it has also created critical security vulnerabilities, particularly in essential but under-resourced projects. This paper examines a sophisticated attack on the XZ Utils project (CVE-2024-3094), where attackers exploited not just code, but the entire open-source development process to inject a backdoor into a fundamental Linux compression library. Our analysis reveals a new breed of supply chain attack that manipulates software engineering practices themselves -- from community management to CI/CD configurations -- to establish legitimacy and maintain long-term control. Through a comprehensive examination of GitHub events and development artifacts, we reconstruct the attack timeline, analyze the evolution of attacker tactics. Our findings demonstrate how attackers leveraged seemingly beneficial contributions to project infrastructure and maintenance to bypass traditional security measures. This work extends beyond traditional security analysis by examining how software engineering practices themselves can be weaponized, offering insights for protecting the open-source ecosystem.

==> TODO.tex <==
\section{TODO}

- Origin of the actor (git commits are in gmt+8, but github events show that most activities was between 10:00 to 19:00 UTC) you can fake git dates, you can also fake github events, but they do not match apparently, there is question about IRC activity. but there are also other places where dattime could be read from to check his activity.

- IRC logs exist but are not public, they may be granted on reasonably requests.

- Dataset should be important part of this, but maybe we can make a interactive-like webapp to show this story timeline in SE perspective. 

- other reported attempts to hijack a project link \url{https://openssf.org/blog/2024/04/15/open-source-security-openssf-and-openjs-foundations-issue-alert-for-social-engineering-takeovers-of-open-source-projects/}

- discussion on how to deal with this situation (ie companies using OSS should donate to OSS money or developers time) \url{https://www.cisa.gov/news-events/news/lessons-xz-utils-achieving-more-sustainable-open-source-ecosystem}

- Developer mental chalange For considerations section \url{https://www.conquer-your-risk.com/2024/04/03/xz-attack-and-cve-2024-3094-a-mental-health-exploitation-of-the-open-source-community/}


"Stress and burnout in open source: toward finding, understanding, and mitigating unhealthy interactions" \url{https://dl.acm.org/doi/abs/10.1145/3377816.3381732}

- Discussion on using automation tools in order to gain credibility on github or other sites.


- nice read on buildtools in xz attack \url{https://felipec.wordpress.com/2024/04/04/xz-backdoor-and-autotools-insanity/}
This is also discussion on technical dept in those build tools that are gargantuan in size because all of the cases they have to check. In those tools there are still checks avalible for edge cases that were true in 1996 but you will not find such edge cases today, but the checks are still available.

- There is a wider discussion going on on going back to Makefile 


- AI-enabled future crime \url{https://link.springer.com/article/10.1186/s40163-020-00123-8}

==> timeline_text.tex <==
- 2021.10.29 first Jia commit \texttt{.editorconfig} \url{https://www.mail-archive.com/xz-devel@tukaani.org/msg00512.html}
- 2021.11.10 Jia propose to change the test framework base on Seatest \url{https://www.mail-archive.com/xz-devel@tukaani.org/msg00514.html}
- 2021.11.12 first Jia review \url{https://www.mail-archive.com/xz-devel@tukaani.org/msg00518.html}
- 2022.05.19 pressure for more maintainer \url{https://www.mail-archive.com/xz-devel\@tukaani.org/msg00562.html}
- 2022.06.07 additional pressure for more maintainers \url{https://www.mail-archive.com/xz-devel\@tukaani.org/msg00566.html}
- 2022.12.12 Jia created the GitHub organization and the GitHub repo for \textit{XZ Utils}.
- 2022.12.12 Jia put his email address as the default contact address \href{https://github.com/tukaani-project/.github/commit/3358b3d9ad3d47774194fef9129a479adaa4a4fc}{3358b3d}
- 2022.12.13 First Jia Release
- 2023.01.11 Jia started to do the announcements on the mailing list \url{https://www.mail-archive.com/xz-devel@tukaani.org/msg00634.html}
- 2024.01.11 Introduction of \texttt{ifunc}
- 2024.01.19 Jia migrated the website to the GitHub page
- Replace the translation process
- 2024.02.23 two ``test files'' that contained the stages of the malicious script are introduced
- 2024.02.24 XZ 5.6.0 is released
- 2024.02.26 commit in CMakeLists.txt that sabotages the Landlock security feature
- 2024.03.04 the backdoor leads to issues with Valgrind
- 2024.03.09 two ``test files'' are updated, CRC functions are modified, Valgrind issue is ``fixed''
- 2024.03.09 XZ 5.6.1 is released
- 2024.03.28 bug is discovered, Debian and RedHat notified
- 2024.03.28 Debian rolls back XZ 5.6.1 to 5.4.5-0.2 version
- 2024.03.28 GitHub accounts of both me (Larhzu) and Jia Tan were suspended. Larhzu was reinstated on 2024-04-02.
- 2024.03.29 an email is published on the OSS-security mailing list
- 2024.03.29 RedHat confirms backdoored XZ was shipped in Fedora Rawhide and Fedora Linux 40 beta
- 2024.03.30 Debian shuts down builds and starts the process of rebuilding it
- 2024.04.02 XZ main developer recognizes the backdoor incident
- 2024.04.30 Redhat release RHEL 9.4
- 2024.06.29 Debian release 12.6
